Interpreting Neural Network Judgments via Minimal, Stable, and Symbolic Corrections

We present a new algorithm to generate minimal, stable, and symbolic corrections to an input that will cause a neural network with ReLU activations to change its output. We argue that such a correction is a useful way to provide feedback to a user when the network's output is different from a desired output. Our algorithm generates such a correction by solving a series of linear constraint satisfaction problems. The technique is evaluated on three neural network models: one predicting whether an applicant will pay a mortgage, one predicting whether a first-order theorem can be proved efficiently by a solver using certain heuristics, and the final one judging whether a drawing is an accurate rendition of a canonical drawing of a cat.

==> pre.tex <==
\section{Preliminaries}
\label{sec:pre}

==> tool.tex <==
\section{Implementation}
\label{sec: tool}
We implemented our approach in a tool called \tool.
%
\tool is written in three thousand lines of Python code.
%
To implement $\funname{findMinimumConcreteCorrection}$, we used a customized version
of the CleverHans library~\cite{cleverhans}.
%
To implement $\funname{isFeasible}$ which checks feasibility of generated linear constraints,
we applied the commercial linear programming solver Gurobi 7.5.2~\cite{gurobi}.
